Exact Simulation of Longitudinal Data from Marginal Structural Models

Simulating longitudinal data from specified marginal structural models is a crucial but challenging task for evaluating causal inference methods and informing study design. While data generation typically proceeds in a fully conditional manner using structural equations according to a temporal ordering, it is difficult to ensure alignment between conditional distributions and the target marginal causal effects, which presents a fundamental challenge. To address this, we propose a flexible and efficient algorithm for simulating longitudinal data that adheres exactly to a specified marginal structural model. Our approach accommodates time-to-event outcomes and extends naturally to survival settings, which are prevalent in applied research. Compared to existing approaches, it offers several advantages: it enables exact simulation from a known causal model rather than relying on approximations; avoids restrictive assumptions about the data-generating process; and remains computationally efficient by requiring only the evaluation of analytical expressions, rather than Monte Carlo methods or numerical integration. Through simulation studies replicating realistic scenarios, we validate the method's accuracy and utility. Our method will facilitate researchers in effectively simulating data with target causal structures for their specific scenarios.

==> appndices/MSM_and_IPTW.tex <==


\subsection{Marginal structural models (MSMs)}

\textcolor{red}{Texts copied from COS need to rewrite!}

Several methods are available to adjust for exposure-affected time-varying confounding. Structural nested models (SNMs), introduced by \cite{robins1989analysis} and \cite{robins1991correcting}, estimate the causal effect of exposure by contrasting mean outcomes under hypothetical exposure scenarios: $\E(Y(a) - Y(0) \cmid A = a, L) = \beta_1 a + \beta_2 L$. When treatments vary over time, the model requires a separate equation for each time point. For two time points, an additive structural nested mean model can be specified with the following equations:
 \begin{align}
     \E[Y(a_0, a_1 = 0) - Y(a_0= 0, a_1 = 0) \cmid A_0 = a_0] &= \beta_0 a_0\\
    \E[Y(a_0, a_1) - Y(a_0, a_1 = 0) \cmid L_1 (a_0) = l_1,A_0 = a_0, A_1(a0) = a_1] &=  \\
    a_1(\beta_11 + \beta_12 l_1 + \beta_13 a_0 + \beta_14 a_0 l_1)
 \end{align}
The ``nested" nature of SNMs comes from specifying one equation for each time point. The first equation models the effect of receiving treatment at time 0 and not thereafter, while the second equation models treatment at time 1, and so on for additional time points. G-estimation is a key approach used with SNMs, identifying parameters that render the exposure variable independent of the counterfactual outcome, assuming conditional exchangeability. For time-to-event outcomes, SNMs include Structural Nested Accelerated Failure Time Models (SNAFTM) \citep{robins1992estimation,hernan2005structural}, and Structural Nested Cumulative Failure Time Models (SNCFTM)  \citep{picciotto2012structural}.

As an alternative to SNMs, Marginal Structural Models (MSMs) have been developed to estimate causal effects of time-varying treatments \citep{robins1997msm,hernan2000marginal}. MSMs model interventional outcomes as a function of treatment history, while marginalizing over post-baseline confounders:
\begin{align*}
    \E[Y \cmid do(\Bar{a}))] = f(\Bar{a};\gamma).
\end{align*}
For survival outcomes, the marginal structure of the outcome can be modeled via hazard, such as using Cox regression \citep{cox1972regression} or an additive hazard model \citep{aalen1989linear}.  A Cox MSM specifies proportional hazard function:
\begin{align*}
    \lambda_{\bar{a}_t} (t) = \lambda_0(t) \exp \left \{ g(\Bar{a_t}; \bs \psi) \right \}
\end{align*}
where $\lambda_0(t)$ is the baseline (e.g.~`never treated') counterfactual hazard at time t, $\bar{a}_t$ denotes the treatment history up to time t. $g(\Bar{a_t}; \psi)$ is a known function describing how treatment influences the hazard. If the hazard function is modified to $ \lambda_{\bar{a}_t} (t) = \lambda_0(t)+ \left \{ g(\Bar{a_t}; \bs \theta) \right \}$, it results in Aalen's additive hazard model.

MSMs are \textit{marginal} because they model causal effects as marginal quantities by averaging over time-varying covariates, and they are \textit{structural} because they explicitly model causal relationships, unlike associational models that capture observational patterns. MSMs can be estimated using methods such as g-computation (g-formula) \citep{robins1986new}, inverse probability of treatment weighting (IPTW), and doubly robust methods such as targeted maximum likelihood estimation (TMLE) \citep{van2006targeted}. A systematic review of the literature \citep{clare2019causal} found that IPTW-estimated MSMs are the most commonly used approach for longitudinal data with time-varying confounding due to their simplicity in both implementation and interpretation..


\subsection{Why simulating from MSMs is challenging}\label{sec:MSM_challenging}

For both method evaluation and sample size calculation, it is essential to be able to simulate data that precisely follows a known causal structure. However, simulating longitudinal data from a pre-specified MSM is not a straightforward task. While it seems \textit{natural} to generate data sequentially -- creating each individual's covariates, treatment status, and survival status at each time point based on past information -- MSMs rely on marginal, rather than conditional models. This makes it difficult to sequentially simulate from conditional models in a way that aligns with a pre-specified marginal model.

To illustrate this, consider the causal model in the DAG shown in Figure \ref{fig:chap4_dag2}. The DAG imposes the following factorization on the joint distribution:
% of $U$,$L_0$,$A_0$,$Y_1$,$L_1$,$A_1$,$Y_2$:
\begin{align*}
    P(U,L_0,A_0,Y_1,L_1,A_1,Y_2) & = P(U)P(L_0 \cmid U) P(A_0 \cmid L_0) P(Y_1 \cmid U,L_0,A_0) \\
    & \cdot P(L_1 \cmid U, L_0,A_0,Y_0) P(A_1 \cmid L_1, A_0, Y_0) P(Y_2 \cmid U,L_1, A_1, Y_1).
\end{align*}

This factorization suggests a straightforward simulation process: first generate the latent variable $U$, then sequentially generate $L_0$ given $U$, $A_0$ given $\{L_0, U\}$, $Y_1$ given $\{U,L_0,A_0)$, followed by the same process for subsequent time points.

% This factorization of the joint distribution immediately suggests a generating process from which it would be straightforward to simulate data that obey a given DAG: choose specific conditional distributions and sequentially generate first the latent variable $U$, then for $t=1$ we simulate $L_0$ given $U$ then, $A_0$ given $\{L_0, U\}$, followed by $Y_1$ given $\{U,L_0,A_0)$, before we move onto the next time point $t=2$ and simulate in a similar order with additional temporal relationship. 
However, if we want this data-generating process to also follow a given MSM that parameterizes $P(Y_1 \mid do(a_0))$ and $ P(Y_2 \mid do(a_0,a_1))$. Applying g-formula yields:
\begin{align}
    P(Y_1 \mid do(a_0)) &= \sum_{l,u}  P(Y_1 \cmid U = u,L_0 = l,A_0 = a_0) P(L_0 = l \cmid U) P(U= u) \label{eqn:chap4_g1} \\ 
    P(Y_2 \mid do(a_0,a_1)) & = \sum_{l_0,l_1,u}  P(Y_2 \cmid U = u,L_1 = l_1, A_1 = a_1, Y_1 = 1)  \nonumber \\ \label{eqn:chap4_g2}
    &P(L_1 = l_1 \cmid U = u, L_0 = l_0, A_0 = a_0, Y_0 = 1) P(L_0 = l_0 \cmid U) P(U= u) 
\end{align}
For continuous variables, these sums are replaced by integrals. Simulating data from given MSMs for $P(Y_1 \mid do(a_0))$ and $P(Y_2 \mid do(a_0,a_1))$ requires compatible choices for all components in Equation (\ref{eqn:chap4_g1}) and (\ref{eqn:chap4_g2}). While this is feasible for linear models, it becomes highly challenging when moving beyond linear relationships -- especially with non-collapsible models like logistic regression or Cox proportional hazards models. This is the core difficulty in simulating data from a pre-specified MSM: finding compatible MSMs and conditional distributions is generally intractable in non-linear settings.
  \centering
\begin{figure}

  \begin{tikzpicture}
  [rv2/.style={rv, inner sep=0.1mm}, node distance=20mm, >=stealth]
  \pgfsetarrows{latex-latex};
\begin{scope}
  \node[rvs0] (Z0) {$L_0$};
  \node[rvs0, below right of=Z0] (X0) {$A_0$};
  \node[rvs0, above right of=X0] (Z1) {$L_1$};
  \node[rvs0, below right of=Z1] (X1) {$A_1$};
  \node[rvs0, below right of=X0, xshift=0mm, yshift=-5mm] (Y1) {$Y_1$};
  \node[rvs0, below right of=X1, xshift=0mm, yshift=-5mm] (Y2) {$Y_2$};
  % \node[right of=Z1] (d1) {$\cdots$};
  % \node[right of=X1] (d2) {$\cdots$};
  \node[lv, above of=Z1, yshift=-5mm] (U) {$U$};
  % \node[rvs0, right of=d1] (ZT) {$L_T$};
  % \node[rvs0, right of=d2] (XT) {$A_T$};
  % \node[rvs0, below right of=XT, xshift=0mm, yshift=-5mm] (YT) {$Y_{T+1}$};

  \draw[degl] (U) to[bend right=10] (Z0);
  \draw[degl] (U) to[bend right=25] (Y1);
  \draw[deg] (Z0) -- (Z1);
  \draw[deg] (Z0) -- (X0);
  \draw[deg] (Z0) to[bend right] (Y1);
  \draw[deg] (X0) -- (Z1);
  \draw[deg] (X0) -- (Y1);
  \draw[deg] (Y1) -- (Z1);
  \draw[deg] (Y1) -- (X1);
  \draw[deg] (Z1) -- (X1);
  \draw[degl] (U) -- (Y2);
  \draw[deg] (X0) -- (X1);
   % \draw[deg, dashed] (C) to[bend right=20] (XT);
   \draw[degl] (U) -- (Z1);
   \draw[deg] (X1) -- (Y2);
  \draw[deg] (Z1) to[bend right] (Y2);
  \draw[deg] (Y1) -- (Y2);
   % \draw[deg] (C) -- (ZT);
   % \draw[deg] (Z1) -- (d1);
   % \draw[deg] (X1) -- (d2);
   % \draw[deg] (d1) -- (ZT);
   % \draw[deg] (d2) -- (XT);
   % \draw[deg] (ZT) -- (XT);   
  % \draw[deg, dashed] (C) to[bend right=-25] (YT);
  % \draw[deg, dashed] (Z1) to[bend left=10] (YT);
  % \draw[deg, dashed] (X1) -- (YT);
  % \draw[deg, dashed] (X0) -- (YT);
    % \draw[deg] (XT) -- (YT);
    % \draw[deg] (ZT) to[bend right] (YT);
  \end{scope}
    \end{tikzpicture}
 \caption{An example DAG showing temporal relationships in a longitudinal discrete setting.}
  \label{fig:chap4_dag2}

\end{figure}

==> appndices/Rcode.tex <==
Here is an example code to simulate data following the setup in Section \ref{sec:soul}. 
\begin{lstlisting}
library(data.table)
library(copula)

sim_func <- function(n = 500, 
                     rho1 = -0.5, rho2 = 2,
                     K = 5, betaS = -0.5,
                     betaB2 = -0.5, betaSB2 = 0.3){
  # copulas
  copL <- tCopula(param = rho1, df = 5, dim = 2, dispstr = "un")
  copW <- normalCopula(param = rho2, dim = 2, dispstr = "un")
  dat <- data.table()
  dat$surv <- rep(1,n)
  
  # baseline vars
  dat[, B1 := rexp(n, rate = 2)]
  dat[, B2 := rbinom(n, size = 1, prob = 0.7)]
  baseline_vars <- c("B1","B2")
  
  # a data table to store calculated quantiles to be carried over to the next time step
  comp_dat <- copy(dat[,baseline_vars, with = F])

  for (k in 0:K){
    n_surv <- sum(dat$surv, na.rm = T)
    if (k>0){
      comp_dat <- comp_dat[Y == 0,]
      if (k > 1){
        comp_dat[,grep("_prev$", colnames(comp_dat), value = TRUE):= NULL]
      }
      # reset names
      setnames(comp_dat,
               old = setdiff(names(comp_dat), baseline_vars),
               new = paste0(setdiff(names(comp_dat), baseline_vars), "_prev"))
    }
    
    # random quantiles
    comp_dat[, paste0("F_L",k,"|surv"):= runif(n_surv)]
    comp_dat[, paste0("F_W",k,"|L",k,"_surv"):= runif(n_surv)]
    comp_dat[, paste0("F_S",k,"|L",k,"_surv"):= runif(n_surv)]
    comp_dat[, paste0("F_Y|LW",k,"_surv"):= runif(n_surv)]
    
    if (k == 0){
      comp_dat[,L := qgamma(get(paste0("F_L",k,"|surv")), shape = 1 + 0.5*B1 + 0.5*B2, scale = 1)]
      comp_dat[,W := qbinom(get(paste0("F_W",k,"|L",k,"_surv")), size = 1, prob = expit(-0.2 +0.5 * B1 + 0.5*B2))]
    } else{
      comp_dat[,L := qgamma(get(paste0("F_L",k,"|surv")), shape = 1 + 0.5*B1 + 0.5*B2 +  0.1 * L_prev  - 0.5 * S_prev, scale = 1)]
      comp_dat[,W := qbinom(get(paste0("F_W",k,"|L",k,"_surv")), size = 1, prob = expit(-0.2 + 0.5 * B1 + 0.5*B2 + W_prev - 0.6* S_prev))]
    }
    
    comp_dat[,S := qbinom(get(paste0("F_S",k,"|L",k,"_surv")),size = 1, prob = expit(-1.5 + 0.5*B1 + 0.5*B2 + 0.5* L + 0.5 * W))]
    
    if (k >0){
      #get the distributions of Ls and Ws in the survivors
      for (j in (1:k)){
        if (j<k){
          comp_dat[,paste0("F_W",k-j,"|L",k-j,"_surv"):= cCopula(as.matrix(cbind(get(paste0("F_Y|L",k-j,"_W", k-j-1,"_surv_prev")),
                                 get(paste0("F_W",k-j,"|L",k-j,"_surv_prev")))),copula = copW)[,2]]
          comp_dat[,paste0("F_L",k-j,"|surv"):= cCopula(as.matrix(cbind(get(paste0("F_Y|LW",k-j-1,"_surv_prev")),
                                get(paste0("F_L",k-j,"|surv_prev")))),copula = copL)[,2]]
        } else{
          comp_dat[,paste0("F_W",k-j,"|L",k-j,"_surv"):= cCopula(as.matrix(cbind(get(paste0("F_Y|L",k-j,"_surv_prev")),
                get(paste0("F_W",k-j,"|L",k-j,"_surv_prev")))),copula = copW)[,2]]
          comp_dat[,paste0("F_L",k-j,"|surv"):= cCopula(as.matrix(cbind(F_Y_surv_prev,
                get(paste0("F_L",k-j,"|surv_prev")))),copula = copL)[,2]]
        }
      }
    }
    
    for (j in (0:k)){
      if (j<k){
        comp_dat[,paste0("F_Y|L",k-j,"_W", k-j-1,"_surv"):= cCopula(as.matrix(cbind(get(paste0("F_W",k-j,"|L",k-j,"_surv")),
        get(paste0("F_Y|LW",k-j,"_surv")))),copula = copW,inverse = T)[,2]]
        comp_dat[,paste0("F_Y|LW",k-j-1,"_surv"):= cCopula(as.matrix(cbind(get(paste0("F_L",k-j,"|surv")),
        get(paste0("F_Y|L",k-j,"_W", k-j-1,"_surv")))),copula = copL,inverse = T)[,2]]
      }else{
        comp_dat[,paste0("F_Y|L",k-j,"_surv"):= cCopula(as.matrix(cbind(get(paste0("F_W",k-j,"|L",k-j,"_surv")),
        get(paste0("F_Y|LW",k-j,"_surv")))),copula = copW,inverse = T)[,2]]
        comp_dat[,F_Y_surv:= cCopula(as.matrix(cbind(get(paste0("F_L",k-j,"|surv")),
        get(paste0("F_Y|L",k-j,"_surv")))),copula = copL,inverse = T)[,2]]
      }
    }
    
    # hazard
    comp_dat[, lambda := exp(-2) *exp(betaS * S + betaB2 * B2 + betaSB2*B2*S)]
    comp_dat[, T := qexp(F_Y_surv, rate = lambda)]
    comp_dat[, Y := 1*(T<1)]
    
    dat[surv == 1, paste0("L","_",k) := comp_dat$L]
    dat[surv == 1, paste0("W","_",k) := comp_dat$W]
    dat[surv == 1, paste0("S","_",k) := comp_dat$S]
    dat[surv == 1, paste0("Y","_",k) := comp_dat$Y]
    dat[surv == 1, T := (comp_dat$T + k)]
    dat[,surv := 1*(get(paste0("Y_",k)) == 0)]
    return(dat)
  }
\end{lstlisting}


==> appndices/competing_risk.tex <==
% \documentclass[a4paper]{article}
% % \usepackage[subpreambles=true]{standalone}
% % \usepackage{import}
% \input{shortcuts_survivl}
% \begin{document}
At each time step $k$, after simulating time-varying covariate $L_k$ and treatment $A_k$, we generate the primary outcome $Y_k$ and a competing risk $D_k$ using their respective auxiliary variables $\Tilde{Y}_k$ and $\Tilde{D}_k$, following the approach outlined in Section \ref{sec:survival}. For brevity, baseline covariates $\bs Z$ continue to be omitted, but in settings where they are present, they can be simulated as the initial step and included in the conditioning set of all subsequent quantities. 

Under this simulation framework, we specify:
\begin{itemize}
 \item A marginal structural model for the primary event: $F^*(\Tilde{Y}_{k+1}\cmid do(\bar{A}_k), Y_k = 0, D_k = 0)$;
    \item A marginal structural model for the competing event: $F^*(\Tilde{D}_{k+1}\cmid do(\bar{A}_k), Y_{k} = 0, D_k = 0)$;
    \item A bivariate copula parameterized by $\Psi_{k+1}$ to model the dependence between the above interventional margins of $\Tilde{Y}_{k+1}$ and $\Tilde{D}_{k+1}$;
    \item Bivariate copulas that `weave' the multivariate dependence between $Y_{k+1}$ and past covariates $\bar{L}_k$, given $do(\bar{A}_k)$, $Y_k = 0$ and $D_k = 0$, parameterized by $\Theta_{k,j}$ for $j = 0,\ldots,k$;
    \item Bivariate copulas that `weave' the multivariate dependence between $\Tilde{D}_{k+1}$ and $\bar{L}_k$ conditional on $\Tilde{Y}_{k+1}$, $do(\bar{A}_k)$, $Y_{k} = 0$ and $D_k = 0$, parameterized by $\Phi_{k,j}$ for $j = 0,\ldots,k$.
\end{itemize}
The joint outcome model $p(\Tilde{y}_{k+1},\Tilde{d}_{k+1} \cmid \bar{l}_k,\bar{a}_k, Y_k = 0, D_k = 0)$ factorizes as follows:

\textbf{Primary event model:}
\begin{align}
    p(\Tilde{y}_{k+1} &\cmid\bar{l}_k,\bar{a}_k, Y_k = 0, D_k = 0) \notag\\
      &= p^*(\Tilde{y}_{k+1}\cmid do(\bar{a}_k), Y_{k} = 0, D_k = 0) \times \notag\\\
      & \prod_{j = 0}^{k} c^*_{\Tilde{Y}_{k+1}, L_{j} \mid \bar{L}_{j-1}, \bar{A}_k, Y_k = 0,D_k = 0}\big\{F(\Tilde{y}_{k+1}\cmid \bar{l}_{j-1},  do(\bar{a}_k), Y_k =0, D_k = 0), \nonumber \\
      & \qquad\qquad\qquad\qquad\qquad\qquad\qquad F(l_j \cmid \bar{l}_{j-1}, do(\bar{a}_{k}), Y_k = 0,D_k = 0) ;\Theta_{k,j}\}. \label{eqn:outcome1_survival_comp}
\end{align}

\textbf{Competing event model:}
\begin{align}
    p(\Tilde{d}_{k+1} &\cmid \bar{l}_k,\bar{a}_k, \Tilde{y}_{k+1}, D_k = 0) \notag\\
      &= p(\Tilde{d}_{k+1}\cmid do(\bar{a}_k), \Tilde{y}_{k+1}, D_k = 0) \times \notag\\\  
      &\prod_{j = 0}^{k} c^*_{\Tilde{D}_{k+1}, L_{j} \mid \bar{L}_{j-1}, \bar{A}_k, \tilde{Y}_{k+1} D_k = 0}\big\{F(d_{k+1}\cmid \bar{l}_{j-1}, do(\bar{a}_k), \tilde{y}_{k+1}, D_k = 0), \nonumber \\
      & \qquad\qquad\qquad\qquad\qquad\qquad\qquad F(l_j \cmid \bar{l}_{j-1},  do(\bar{a}_{k}), \tilde{y}_{k+1},D_k = 0) ;\Phi_{k,j}\}. \label{eqn:outcome2_survival_comp}
\end{align}

The first term in (\ref{eqn:outcome2_survival_comp}), the distribution of $\Tilde{d}_{k+1} \cmid \bar{l}_k,\bar{a}_k, \Tilde{y}_{k+1}, D_k = 0$ can be obtained through:
$$F(\Tilde{d}_{k+1} \cmid \bar{l}_k,\bar{a}_k, \Tilde{y}_{k+1}, D_k = 0)  = h \big \{F*(\Tilde{d}_{k+1} \cmid \bar{l}_k,\bar{a}_k, Y_k =0, D_k = 0), F^*(\Tilde{y}_{k+1} \cmid \bar{l}_k,\bar{a}_k, Y_k =0, D_k = 0) \big \}.$$ 
The challenge lies in computing $F(l_j \cmid \bar{l}_{j-1}, do(\bar{a}_{k}), Y_{k} = 0,D_k = 0)$ in (\ref{eqn:outcome1_survival_comp}), and $F(l_j \cmid \bar{l}_{j-1}, do(\bar{a}_{k}), \tilde{y}_{k+1},D_k = 0)$ in (\ref{eqn:outcome2_survival_comp}), for $j = 0, \ldots, k$. The former can be calculated in the same iterative fashion as described in Section \ref{sec:survival}. The latter can be derived as:
\begin{align}
    F(l_j \cmid \bar{l}_{j-1},  do(\bar{a}_{k}), \tilde{y}_{k+1},D_k = 0) &= h \big \{F(l_j \cmid \bar{l}_{j-1}, do(\bar{a}_{k}), Y_k = 0,D_k = 0),\notag\\
    & \qquad F(\tilde{y}_{k+1} \cmid \bar{l}_{j-1},  do(\bar{a}_{k}), Y_k = 0,D_k = 0); \Theta_{k,j} \big \} \label{eqn:outcome_survival_comp2}.
\end{align}

Notably, the two components in the $h$-function in (\ref{eqn:outcome_survival_comp2}) exactly correspond to the those in the primary event model in (\ref{eqn:outcome1_survival_comp}), except with the order of conditioning swapped. Since these values are computed during the simulation of $\Tilde{y}_{k+1}$, requiring only $k+1$ additional evaluations of the $h$-functions in (\ref{eqn:outcome_survival_comp2}). 
% Once these quantiles of $\bar{l}_k$'s are calculated, we apply a very similar procedure to simulating the primary event, the competing event is simulated analogously to the primary event, effectively `unweaving' the pair-copulas linking $\bar{L}_k$ and $D_{k+1}$. 

The algorithm for simulating each time step $k$ for an individual can be summarized into:
\begin{enumerate}
    \item Simulate the time-varying confounder $L_k$ and treatment $A_k$ from their respective distributions.
    \item Compute $F(l_j \cmid \bar{l}_{j-1}, do(\bar{a}_{k}), Y_k = 0,D_k = 0)$ for $j = 0, \dots, k-1$.
    \item Compute $F(y_{k+1}\cmid \bar{l}_{j-1}, do(\bar{a}_k), Y_k =0, D_k = 0)$ for $j = 1,\dots k$, leading to $ u_{k+1} = F(\Tilde{y}_{k+1}\cmid z, do(\bar{a}_k), Y_k =0, D_k = 0)$.
    \item Compute: $\Tilde{y}_{k+1} =F^{*-1}_{\Tilde{Y}_{k+1}\cmid do(\bar{A}_k), Y_k =0, D_k = 0}(u_{k+1}\cmid do(\bar{a}_k), Y_k =0, D_k = 0)$.
    \item Compute $F(l_j \cmid \bar{l}_{j-1}, do(\bar{a}_{k}), \Tilde{y}_{k+1},D_k = 0)$ for $j = 0,\ldots, k$ by evaluating $k+1$ $h$-functions following (\ref{eqn:outcome_survival_comp2}).
    \item Compute $F(\Tilde{d}_{k+1}\cmid \bar{l}_{j-1}, do(\bar{a}_k), \Tilde{y}_{k+1} =0, D_k = 0)$ for $j = 1,\ldots k$, leading to $v_{k+1} = F(\Tilde{d}_{k+1}\cmid do(\bar{a}_k), \Tilde{y}_{k+1}, D_k = 0)$.
    \item Compute: $\Tilde{d}_{k+1} =  F_{\Tilde{D}_{k+1}\cmid do(\bar{A}_k), \Tilde{Y}_{k+1}, D_k = 0}^{*-1}(\Tilde{d}_{k+1}\cmid do(\bar{a}_k), \Tilde{y}_{k+1}, D_k = 0)$.

\end{enumerate}
This approach requires at most $4k + 7$ evaluations of analytic functions per individual per time step. An example implementation is available at \href{https://github.com/XiLinStats/LongSiMSM}{\texttt{https://github.com/XiLinStats/LongSiMSM}}.

% \end{document}

==> appndices/details_simulation.tex <==
\textbf{Models for baseline, time-varying covariates and treatment}

A baseline:
\begin{align*}
    B \sim \Exp(2) &&  L_0 \sim  \operatorname{Gamma}(k = 1 + 0.5 \,B + 0.5\,C, \; \theta =1)\\
   C \sim \Bernoulli(0.7)  && W_0 \sim \Bernoulli(\expit\{-0.2+0.5\,B + 0.5\,C\}).
\end{align*}
We specify that throughout the treatment assignment is influenced by $B$, $C$, $L_k$ and $W_k$ as: 
\begin{align*}
       A_k \sim \Bernoulli(\expit\{-1.5+0.5\,B + 0.5\,C + 0.5 \,L_k + 0.5\,W_k\}).
\end{align*}
For subsequent follow-up visits $k > 0$:
\begin{align*}
    L_k &\sim  \operatorname{Gamma}(k = 1 + 0.5 \,B + 0.5\,C + 0.1 \,L_{k-1} - 0.5 \,A_{k-1}, \; \theta =1)\\
    W_k &\sim \Bernoulli(\expit\{-0.2+0.5\,B + 0.5\,C + W_{k-1} - 0.6 \, A_{k-1}\}).
\end{align*}

\textbf{Parameter Scenarios}

Table\ref{tab:demo2_scenarios} summarizes the parameter values for treatment effect size and confounding scenarios:


\begin{table}[ht]
\centering
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{ll}
\toprule
% \textbf{Scenario} & \textbf{Description} \\ 
\midrule
\multicolumn{2}{l}{\textbf{Effect size}} \\
\midrule
\textbf{Large} & $(\beta_A,\beta_{CA}) = (-0.5,0.3) $ \\
\textbf{Small} & $(\beta_A,\beta_{CA}) = (0.2,0.1) $ \\

\midrule
\multicolumn{2}{l}{\textbf{Level of confounding}} \\
\midrule
\textbf{High} &  $(\rho_L,\rho_W) = (0.9 ,0.7) $ \\
\textbf{Medium} & $(\rho_L,\rho_W) = (-0.5,0.4) $\\
\textbf{Low} & $(\rho_L,\rho_W) = (-0.1,-0.2) $\\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{Parameter values of treatment effect size and confounding scenarios.}
\label{tab:demo2_scenarios}
\end{table}

\textbf{Runtime details}

% The proposed algorithm, as previously discussed, exclusively relies on evaluating analytic functions, making it highly efficient. 
Table \ref{tab:runtime} reports the runtime required to simulate data under the setup for the large causal effect with  medium confounding scenario. The simulations were carried out on a local laptop using a single score without parallelization. Generating data for $n$ up to 10,000 units takes only a few seconds, while even for a very large sample size ($n = 50,\!000$) and 11 time steps ($K= 10$), the runtime remains under one minute. This computational efficiency is crucial for tasks such as method evaluation and sample size calculations in clinical trial design, where simulations must be repeated across various parameter values. For example, determining the sample size might require testing 10 different parameter combinations (such as effect sizes, prevalence of drop-in treatments, or adherence levels) across four sample sizes, each bootstrapped 200 times to estimate statistical power. This requires $10\times 4 \times 200 = 8,\!000$ simulations. Using our method, suppose $n = 10,000$ and $K=10$, the total runtime is approximately 13 hours on a single core, which can be reduced to about 2 hours using an 8-core laptop or under 10 minutes on a 50-core CPU through parallelization. 

In contrast, simulation methods requiring computationally intensive operations, such as Monte Carlo approximations \citep[see, for example,][]{seaman2023simulating} or numerical integration, are often too slow to support such large-scale simulations. This highlights a key advantage of our proposed method: its ability to handle extensive simulation demands efficiently, making it well-suited for practical applications.



% \begin{table}[ht]
% \centering
% \begin{adjustbox}{max width=\textwidth}
% \begin{tabular}{rrr}
% \toprule
% \multicolumn{1}{c}{$n$} & \multicolumn{1}{c}{$K = 5$} & \multicolumn{1}{c}{$K = 10$} \\
% \midrule
% 1,000  & 0.27  & 0.79  \\
% 2,000  & 0.45  & 1.68  \\
% 5,000  & 1.69  & 2.49  \\
% 10,000 & 2.70  & 6.09  \\
% 50,000 & 16.50 & 45.49 \\
% \bottomrule
% \end{tabular}
% \end{adjustbox}
% \caption{Runtime (in seconds) to simulate a dataset of size $n$, averaged over 20 repeats.}
% \label{tab:runtime}
% \end{table}

\textbf{Weight calculation}

To fit the Cox marginal model, we employ stabilized inverse probability of treatment weighting, with weights for subject $i$ at time step $k$ calculated as:
\begin{align*}
    \prod_{j=0}^k \frac{\hat{p}_j(A_j \mid C, \bar{A}_{j-1}, Y_j = 0)}{\hat{p}_j(A_j \mid B, C, \bar{L}_j,\bar{W}_j, \bar{A}_{j-1}, Y_j = 0)},
\end{align*}
where $\hat{p}_j(A_j \mid C, \bar{A}_{j-1}, Y_j = 0)$ and $\hat{p}_j(A_j \mid B, C, \bar{L}_j,\bar{W}_j, \bar{A}_{j-1}, Y_j = 0)$ are estimated using logistic regression models fitted to the survivors at time step $j$. 

    The denominator in the weight formula represents the correctly specified propensity score model under the assumed data-generating process, while the numerator stabilizes the weights. To avoid unintended confounding, the baseline covariates included in the numerator must also be adjusted for in the marginal structural model \citep{cole2008constructing}. In accordance with the model in (\ref{eqn:sim_MSM}), we only include $C$ in the numerator for stabilization.

==> sections/appendices.tex <==

\subsection{Simulate \protect\((L_2,A_2,Y_3 \cmid Z,\bar{L}_1,\bar{A}_1, Y_2 = 0)\protect\)}

We simulate $(L_2,A_2)$ given $\cmid Z,\bar{L}_1,\bar{A}_1, Y_2 = 0)$ similarly to the previous time step k=1, here we put more focus on simulating $Y_3$ and the copula $ c^*_{Y_3 \bar{L}_2\mid \bar{A}_1, Z}(u^*_{Y_1},u_{L_0},u_{L_1}; \bs \theta)$.
\begin{align}
    p(l_2,a_2,y_3 \cmid z, \bar{l}_1, \bar{a}_1)  &=  p_{L_2\mid Z,\bar{L}_1,\bar{A}_1} (l_2 \cmid z,\bar{l}_1, \bar{a}_1) \cdot 
    p_{A_2 \mid Z,\bar{L}_2,\bar{A}_1}(a_2 \cmid z,\bar{l}_2, \bar{a}_1) \label{eqn:k_2_past}\\
    &\cdot p_{Y_3\mid \bar{A}_2,Z}^*(y_3\cmid do(\bar{a}_2),z)\\
    &\cdot c^*_{Y_3 \bar{L}_2\mid \bar{A}_2, Z}(u^*_{Y_3},u_{L_0},u_{L_1},u_{L_2}; \bs \theta) \label{eqn:k_2_cop},
\end{align}
where we use a pair-copula construction as depicted in Figure \ref{fig:pcc_k_2_cop} for the four-dimensional copula in (\ref{eqn:k_2_cop}). Since there many possible D-vine PCCs for this given copula, where we can rearrange the positions of the four variables, we recommend the specific PCC shown in Figure \ref{fig:pcc_k_2_cop}. This choice is advantageous because the inputs into the pair-copula that do not involve $Y_3$, including the quantiles of $F_{L_1\mid L_0}$ and $F_{L_2\mid L_0,L1}$, are readily available and correspond directly to the uniform random variables $w$'s used to sequentially generate the $L_k$'s. Compared to other orderings of the variables,  this particular D-vine PCC offers the convenience of using the pre-generated uniform variables without the need to compute additional input quantiles for the copulas.


\begin{figure}
    \centering
    \begin{tikzpicture}
    
  % First row
    \node[circle, draw, minimum size = 1cm, ] (1) {$L_2$};
    \node[circle, draw, minimum size = 1cm, right=2cm of 1] (2) {$L_1$};
    \node[circle, draw, minimum size = 1cm, , right=2cm of 2] (3) {$L_0$};
    \node[circle, draw, minimum size = 1cm, , right=2cm of 3] (4) {$Y_3$};
    \node[  minimum size = 1cm , right=2cm of 4] (T1) {$T_1$};

    \draw (1) -- node[above] {$L_1 L_2$} (2);
    \draw (2) -- node[above] {$L_0 L_1$} (3);
    \draw (3) -- node[above] {$L_0 Y_3$} (4);

  % Second row
    \node[circle, draw, minimum size = 1cm, below right =1cm and 1cm of 1] (12) {$L_1 L_2$};
    \node[circle, draw, minimum size = 1cm, below right =1cm and 1cm of 2] (23) {$L_0 L_1$};
        \node[circle, draw, minimum size = 1cm, below right =1cm and 1cm of 3] (34) {$L_0 Y_3$};
    \node[  minimum size = 1cm , below=1cm of T1] (T2) {$T_2$};
    \draw (12) -- node[above] {$L_0L_2\mid L_1$} (23);
    \draw (23) -- node[above] {$L_1Y_3\mid L_0$} (34);
  
  % Third row
  \node[circle, draw, minimum size = 0.8cm, below right =1cm and 1cm of 12] (13_2) {\tiny $L_0 L_2 \mid L_1$};
  \node[circle,draw, minimum size = 1cm, below right =1cm and 1cm of 23]  (24_3) {\tiny $L_1 Y_3 \mid L_0$};
    \node[  minimum size = 1cm , below=1cm of T2] (T3) {$T_3$};
  \draw (13_2) -- node[above] {\small $L_2 Y_3 \mid \bar{L}_1$} (24_3);
  
\end{tikzpicture}
    \caption{A D-vine PCC of $c^*_{Y_3 \bar{L}_2\mid \bar{A}_2, Z}$ in (\ref{eqn:k_2_cop}).  Note that all the copulas in this figure are conditioned on $do(\bar{A}_2)$, $Z$ and $Y_2 =0$ but these conditioning variables are omitted for brevity.}
    \label{fig:pcc_k_2_cop}
\end{figure}

The steps to simulate from this factorization are as follows:
\begin{enumerate}[label=(\roman*)]
    \item Generate three uniform random numbers $w_7,w_8,w_{9}$.
    \item Simulate $(l_2,a_2)$ sequentially according to (\ref{eqn:k_2_past}):
        \begin{enumerate}
            \item $l_2 = F^{-1}_{L_2\mid Z,\bar{L}_1,\bar{A}_1} (w_7 \cmid z,\bar {l}_1,\bar {a}_1) $
            \item $a_2 = F^{-1}_{A_2 \mid Z,\bar{L}_2,\bar{A}_1}(w_8 \cmid z,\bar {l}_2,\bar {a}_1)$
        \end{enumerate}
    \item Simulate the marginal quantile of $Y_2$ from the copula in (\ref{eqn:k_2_cop}) following the PCC shown in Figure \ref{fig:pcc_k_2_cop}: 
    \begin{enumerate}
        \item Starting from Tree 3, first simulate $C_{Y_3\mid L_0L_1}$ from the copula $c^*_{L_2 Y_3 \mid L_0L1}$
            \begin{align}
                 C_{Y_3\mid \bar{L}_1}(u^*_{Y_3} \cmid u_{L_0},u_{L_1}) &= h^{-1}(w_{9}, F_{L_2\mid \bar{L}_1}(l_2\cmid \bar{l}_1)); \bs \theta_{31})\\
                 & = h^{-1}(w_{9}, w_7; \bs \theta_{31}),
            \end{align}
            where $w_7 =F_{L_2\mid \bar{L}_1}(l_2\cmid \bar{l}_1)$ by design as $L_2$ was simulated in step (ii)(a) using this conditional distribution.
        \item Then, in Tree 2, simulate $C_{Y_3\mid L_0}$ from the copula 
        $c^*_{L_1 Y_3 \mid L_0}$:
            \begin{align}
                 C_{Y_3\mid L_0}(u^*_{Y_3} \cmid u_{L_0}) &= h^{-1}( C_{Y_3\mid \bar{L}_1}, F_{L_1\mid L_0}(l_1\cmid l_0)); \bs \theta_{22})\\
                 & = h^{-1}(C_{Y_3\mid \bar{L}_1}, w_4; \bs \theta_{22}),
            \end{align}
        \item in Tree 1, simulate the marginal quantile $u^*_{Y_3}$ from the copula $c^*_{L_0 Y_3}$:
            \begin{align}
             u^*_{Y_3} &= h^{-1}( C_{Y_3\mid L_0}, F_{L_0}(l_0); \theta_{12})\\
             &= h^{-1}( C_{Y_3\mid L_0}, w_1; \theta_{13})
        \end{align}
    \end{enumerate}

    \item Invert the MSM CDF to obtain $y_3$:
        \begin{align*}
            y_3 =  F_{Y_3\mid \bar{A}_2, Z}^{*-1}(u^*_{Y_3}\cmid do(\bar{a}_2),z).
        \end{align*}
\end{enumerate}




\begin{landscape} % Start landscape mode

\begin{figure}
    \centering
    \begin{tikzpicture}
    
  % First row
    \node[circle, draw, minimum size = 1.5cm, ] (1) {$L_k$};
    \node[circle, draw, minimum size = 1.5cm, right=2cm of 1] (2) {$L_{k-1}$};
    \node[circle, draw, minimum size = 1.5cm, , right=2cm of 2] (3) {$L_{k-2}$};
    % \node[circle, draw, minimum size = 1cm, , right=2cm of 3] (4) {$L_{k-3}$};
    \node[circle, minimum size = 1.5cm, , right=0.5cm of 3] (dots1) {$\cdots$};
        \node[circle, draw, minimum size = 1.5cm, , right=0.5cm of dots1] (4) {$L_2$};
    \node[circle, draw, minimum size = 1.5cm, , right=2cm of 4] (5) {$L_1$};
    \node[circle, draw, minimum size = 1.5cm, , right=2cm of 5] (6) {$L_0$};
    \node[circle, draw, minimum size = 1.5cm, , right=2cm of 6] (7) {$Y_{k+1}$};
    \node[  minimum size = 1cm , right=2cm of 7] (T1) {$T_1$};

    \draw (1) -- node[above] {$L_k L_{k-1}$} (2);
    \draw (2) -- node[above] {$L_{k-1} L_{k-2}$} (3);
    \draw (3) -- node[above] {} (dots1);
     % \draw (4) -- node[above] {} (dots1);
      \draw (dots1) -- node[above] {} (4);
       \draw (4) -- node[above] {$L_2L_1$} (5);
    \draw (5) -- node[above] {$L_1 L_0$} (6);
    \draw (6) -- node[above] {$L_0 Y_{k+1}$} (7);

  % Second row
    \node[circle, draw, minimum size = 1.5cm, below right =1cm and 1cm of 1,label= below:$L_k L_{k-1}$] (21) {$\Theta_{2,1}$};
    \node[circle, draw, minimum size = 1.5cm, below right =1cm and 1cm of 2,label= below:$L_{k-1} L_{k-2}$] (22) {$\Theta_{2,2}$};
    \node[circle, minimum size = 1.5cm, , below right =1cm and -0.5cm of dots1] (dots2) {$\cdots$};
    \node[circle, draw, minimum size = 1.5cm, below right =1cm and 1cm of 4,label= below:$L_1L_2$] (23) {$\Theta_{2,{k-1}}$};

    \node[circle, draw, minimum size = 1.5cm, below right =1cm and 1cm of 5,label= below:$L_1 L_0$] (24) {$\Theta_{2,k}$};
    \node[circle, draw, minimum size = 1.5cm, below right =1cm and 1cm of 6,label= below:$L_0 Y_{k+1}$] (25) {$\Theta_{2,k+1}$};
    
    \node[  minimum size = 1cm , below=1.3cm of T1] (T2) {$T_2$};
    \draw (21) -- node[above] {$L_kL_{k-2}\mid L_{k-1}$} (22);
    \draw (22) -- node[above] {} (dots2);
    \draw (dots2) -- node[above] {} (23);
    \draw (23) -- node[above] {$L_2L_0\mid L_1$} (24);
    \draw (24) -- node[above] {$L_1Y_{k+1}\mid L_0$} (25);
  
  % Third row

    \node[circle, draw, minimum size = 1.5cm, below right =1cm and 1cm of 21,label= below:$L_k L_{k-2} \mid L_{k-1}$] (31) {$\Theta_{3,1}$};
    \node[circle, minimum size = 1.5cm, , below right =1cm and -0.5cm of dots2] (dots3) {$\cdots$};
    \node[circle, draw, minimum size = 1.5cm, below right =1cm and 1cm of 23,label= below:$L_2L_0 \mid L_1$] (32) {$\Theta_{3,k-1}$};
    \node[circle, draw, minimum size = 1.5cm, below right =1cm and 1cm of 24,label= below:$L_1Y_{k+1} \mid L_0$] (33) {$\Theta_{3,k}$};
    \node[  minimum size = 1cm , below=1.3cm of T2] (T3) {$T_3$};
  \draw (31) -- node[above] {} (dots3);
    \draw (dots3) -- node[above] {} (32);
    \draw (32) -- node[above] {\small $L_2 Y_{k+1}  \mid \bar{L}_1$} (33);

    % Forth row
    \node[circle, draw, minimum size = 1.5cm, below left =1cm and 1cm of 33,label= below:$L_2 Y_{k+1} \mid \bar{L}_1$] (41) {$\Theta_{4,{k-1}}$};
    \node[  minimum size = 1cm , left=1cm of 41] (40) {};
    \node[  minimum size = 1cm , below=1.3cm of T3] (T4) {$T_4$};

    \draw (40) -- node[above] {} (41);
    
    % Sixth row
    \node[circle, draw, minimum size = 1.5cm, below left =1cm and 1cm of 41,label= below:$L_3 Y_{k+1} \mid \bar{L}_2$] (51) {$\Theta_{5,{k-2}}$};
    \node[  minimum size = 1cm , left=1cm of 51] (50) {};
    \node[  minimum size = 1cm , below=1.3cm of T4] (T5) {$T_5$};

    \node[circle, minimum size = 1.5cm, below left =1cm and 1cm of 51] (61) {$\dots$};
    \draw (50) -- node[above] {} (51);

    % % Fifth row
    % \node[circle, draw, minimum size = 1.5cm, below left =1cm and 1cm of 41,label= below:$L_3 Y_{k+1} \mid \bar{L}_2$] (51) {$\Theta_{5,{k-2}}$};

    % % Sixth row
    % \node[circle, draw, minimum size = 1.5cm, below left =1cm and 1cm of 51,label= below:$L_4 Y_{k+1} \mid \bar{L}_3$] (61) {$\Theta_{6,{k-3}}$};

    % Final row
    % \node[circle, minimum size = 1.5cm, below left =1cm and 1cm of 61] (71) {$\dots$};

    %     % Final row
    \node[circle, draw, minimum size = 1.5cm, below left =1cm and 1cm of 61,label= below:$L_k Y_{k+1} \mid \bar{L}_{k-1}$] (71) {$\Theta_{k+2,1}$};
    \node[  minimum size = 1cm , below=2.5cm of T5] (Tk) {$T_{k+2}$};
        % \node[circle, draw, minimum size = 1.5cm, below left =1cm and 1cm of 51,label= below:$L_k Y_{k+1} \mid \bar{L}_{k-1}$] (71) {$\Theta_{6,{k-3}}$};
    
\end{tikzpicture}
    \caption{A D-vine PCC of $c^*_{Y_3 \bar{L}_2\mid \bar{A}_2, Z}$ in (\ref{eqn:k_2_cop}).  Note that all the copulas in this figure are conditioned on $do(\bar{A}_2)$, $Z$ and $Y_2 =0$ but these conditioning variables are omitted for brevity.}
    \label{fig:pcc_k_2_cop}
\end{figure}


\end{landscape} % End landscape mode


==> sections/illustration.tex <==
% \subsection{Demonstration 1}
We first demonstrate our simulation method with an example replicating the setting in \cite{bodnar2004marginal}, which examines the causal effect of iron supplement use during pregnancy on the odds of anemia at delivery.

Participants are initially randomized into treatment and control groups and are followed up in four visits leading up to delivery. Like the Iron Supplementation Study analyzed in \cite{bodnar2004marginal}, we assume that the participants adhere to their randomly assigned treatment up to $T=3$, after which the standard clinical protocol applies.

We consider baseline variables $\bs Z =\{$B = Pre-pregnancy obesity, C = Age$\}$ and time-varying covariate $L$ = $\{$Hemoglobin level (g/dL)$\}$. The time-dependent treatment, $A_k$, indicates whether an iron supplement is prescribed. The outcome $Y$ is measured at delivery and $Y=1$ indicates an\ae mia at delivery.

The distribution of baseline variables is:
\begin{align*}
    B &\sim \Bernoulli(0.1) && C \sim U(25,\,35)\\
    L_0 &\sim N(11 -0.05\,B -0.02\, C, \,0.5) && A_0 \sim \Bernoulli(0.5).
\end{align*}
For subsequent follow-up visits $k > 0$ we have $L_k \sim N(L_{k-1} + 0.5\,A_{k-1},\,0.1)$, and $A_2 = A_1 = A_0$ with $A_k \sim \Bernoulli(\expit(10 -L_k + 0.1\,A_{k-1}))$ for $k = 3,4$.
% \begin{align*}
%      && \\
%     A_2 &= A_1 = A_0 && A_k \sim \Bernoulli(\expit(10 -L_k + 0.1\,A_{k-1})) \text{ for } k = 3,4.
% \end{align*}
We choose a logistic model for a discrete-time hazard marginal structural model:
\begin{align*}
\Pr[Y = 1\cmid do(\Bar{A}_4),B,C] = \expit(-2 + 0.1\,B + 0.02 \,C - \beta \, \operatorname{cum}(\Bar{A}_4)),
\end{align*}
where $\operatorname{cum}(\Bar{A}_4) = \Sigma_{i=1}^{4}A_i$. This assumes $\exp(\beta)$ as the causal odds ratio of anemia for an incremental dose. If all women receive iron supplements at all four visits, the causal odds ratio would be $\exp(4\beta)$, representing the true value for the ``always treated” efficacy estimand.

We use a t-copula $T_{\rho,\operatorname{df}}$ (with $\rho = -0.5$ and $\operatorname{df}=5$) across all pair-copula construction components to model the dependency between $Y$ and each of $L_0, L_1,L_2,L_3$, and $L_4$. Compared to a Gaussian copula, the t-copula allows for heavier-tailed dependency, capturing stronger associations in the tails. In our example, t-copulas reflect the likelihood that extreme Hb levels (e.g., severely low) are more strongly associated with extreme outcomes (anemia at delivery). This dependency structure may better reflect the underlying association than a Gaussian copula. Our algorithm offers full flexibility, allowing users to choose any copula family and specify different parameters for each bivariate copula in the pair-copula construction.
% \begin{rmk}
%     \red{Add an intuitive interpretation of the parameters and conditional independence here}
% \end{rmk}


We simulated scenarios with varying causal coefficients $\beta = \{-0.5,-0.3,0 \}$, representing strong, moderate and no effect, respectively and considered different samples size $n = \{500,1000,2000\}$. For each combination of $\beta$ and $n$ we generated 400 datasets. We fitted the model $Y = \expit(\alpha + \gamma \,B + \theta \,C - \beta \, \operatorname{cum}(\Bar{A}_4))$ using two approaches: with stablized inverse probability of treatment weights, and an unweighted approach. For each fit, we computed 95\% confidence intervals for $\beta$ using two methods: (1) the robust sandwich estimator of the variance, with rationale provided by \cite{hernan2000marginal} that the use of weights induces within-subject correlation, and (2) non-parametric bootstrap, constructing 95\% confidence intervals from the 2.5\% and 97.5\% percentiles from 200 bootstrap samples. 

Table \ref{tab:demo1_bias} presents the bias with corresponding Monte Carlo standard errors. The inverse-probability-weighted estimator shows minimal bias, with Monte Carlo standard errors decreasing as sample size increases.In contrast, the unweighted estimator remains significantly biased across sample sizes, showing no convergence. Table \ref{tab:demo1_cov} reports coverage rates. Both the sandwich and bootstrap CIs approach 95\% coverage, though with minor under-coverage.  The unweighted estimator, however, exhibits poor coverage due to significant bias in $\beta$. Table \ref{tab:demo1_power} shows the statistical power of the test of treatment effect (null hypothesis: $\beta = 0$) for each estimator, with power of the weighted estimator increasing as the causal effect size and sample size grow. In summary, these results confirm that data generated using our simulation algorithm accurately reflect the intended causal effects.

\begin{table}[h!]
    \begin{center}
         \begin{tabular}{cc cc}
        \toprule
        $\beta$ & $n$ & \textbf{IPTW} & \textbf{Unweighted} \\
        \midrule
        $-$0.5 & 500  & 0.027 (0.186) & 0.270 (0.115) \\
             & 1000 & 0.012 (0.140) & 0.269 (0.079) \\
             & 2000 & 0.009 (0.096) & 0.274 (0.055) \\
        \midrule
        $-$0.3 & 500  & 0.015 (0.179) & 0.236 (0.103) \\
             & 1000 & 0.004 (0.119) & 0.234 (0.073) \\
             & 2000 & 0.009 (0.088) & 0.235 (0.051) \\
        \midrule
         0   & 500  & 0.017 (0.138) & 0.189 (0.083) \\
             & 1000 & 0.015 (0.087) & 0.188 (0.059) \\
             & 2000 & 0.014 (0.072) & 0.193 (0.043) \\
        \bottomrule
    \end{tabular}
    \caption{Bias and Monte Carlo standard errors  (in parentheses, defined as $sd(\hat{\beta})$) for inverse-probability-of-treatment-weighted (`IPTW') and unweighted estimators (`unweighted') across different $\beta$ and $n$ values.}
    \label{tab:demo1_bias}
    \end{center}
   
\end{table}

\begin{table}[h!]
    \centering
    \begin{tabular}{rr ccc c}
        \toprule
        \multicolumn{1}{c}{$\beta$} & \multicolumn{1}{c}{$n$} & \multicolumn{2}{c}{\textbf{IPTW}} & \textbf{Unweighted} \\
        \cmidrule(lr){3-4}
               &     & \textbf{Sandwich} & \textbf{Bootstrap} & \\
        \midrule
        $-0.5$ & 500  & 91.8\% & 93.0\% & 31.8\% \\
             & 1000 & 92.0\% & 91.8\% & 7.5\%  \\
             & 2000 & 92.3\% & 92.8\% & 0.0\%  \\
        \midrule
        $-0.3$ & 500  & 91.0\% & 91.5\% & 35.3\% \\
             & 1000 & 94.3\% & 92.5\% & 8.0\%  \\
             & 2000 & 94.3\% & 93.8\% & 0.3\%  \\
        \midrule
         0.0   & 500  & 92.8\% & 93.0\% & 41.8\% \\
             & 1000 & 95.5\% & 94.3\% & 12.0\% \\
             & 2000 & 92.8\% & 90.0\% & 0.5\%  \\
        \bottomrule
    \end{tabular}
    \caption{Coverage of 95\% confidence intervals for  IPTW-sandwich, IPTW-bootstrap, and unweighted estimators across scenarios with varying $\beta$ and $n$ values.}
        \label{tab:demo1_power}
    \label{tab:demo1_cov}
\end{table}

\begin{table}[h!]
    \centering
    \begin{tabular}{rr ccc c}
        \toprule
        \multicolumn{1}{c}{$\beta$}  & \multicolumn{1}{c}{$n$} & \multicolumn{2}{c}{\textbf{IPTW}} & \textbf{Unweighted} \\
        \cmidrule(lr){3-4}
               &     & \textbf{Sandwich} & \textbf{Bootstrap} & \\
        \midrule
        $-0.5$ & 500  & 83.3\% & 79.5\% & 55.3\% \\
             & 1000 & 97.5\% & 97.8\% & 82.5\% \\
             & 2000 & 100.0\% & 100.0\% & 98.3\% \\
        \midrule
        $-0.3$ & 500  & 45.8\% & 43.0\% & 12.0\% \\
             & 1000 & 80.0\% & 77.8\% & 15.3\% \\
             & 2000 & 95.8\% & 96.5\% & 26.8\% \\
        \midrule
         0.0   & 500  & 7.3\%  & 7.0\%  & 58.3\% \\
             & 1000 & 4.5\%  & 5.8\%  & 88.0\% \\
             & 2000 & 7.3\%  & 10.0\% & 99.5\% \\
        \bottomrule
    \end{tabular}
    \caption{Statistical power to reject the null hypothesis $\beta = 0$; that is, no causal effect.}
\end{table}





% \subsection{Demonstration 2: Sample Size Calculation with Treatment Discontinuity}

% We demonstrate the utility of our simulation method in aiding sample size calculation for trials with complex time-varying treatment. This example, inspired by the contexts of \cite{ryan2024long} and \citep{jastreboff2022tirzepatide},  examines the long-term weight loss effects of the GLP-1 receptor agonists semaglutide and tirzepatide, commonly used in obesity management.

% Our data generating model is loosely based on the SELECT Trial \citep{lincoff2023semaglutide,ryan2024long}, simulating a randomized controlled trial with participants assigned either to a semaglutide treatment arm or a placebo arm. The primary outcome is the percentage reduction in weight after 208 weeks, with participants visiting the study doctor quarterly over a 2-year period.

% Treatment adherence is a critical factor. Gastrointestinal side effects such as nausea, diarrhea, abdominal pain, and vomiting are common with GLP-1 receptor agonists. \cite{jastreboff2022tirzepatide} reported that around  80\% of tirzepatide-treated participants experienced at least one adverse event, with varying severity. Serious events may lead to temporary or permanent discontinuation, as in the SELECT trial where 16.6\% of participants discontinued due to adverse effects \citep{ryan2024long}. Accounting for this non-negligible adherence issue is essential for accurate sample size calculations. 

% The baseline variables in our model are $\bs Z =\{$ B = BMI, S = Sex, C= Age $\}$ and time-varying covariate $L$ = $\{$Degree of gastrointestinal reaction$\}$. These variables were selected based on findings that the difference in mean weight reduction between the treatment and placebo arms varies by BMI, sex, and age, and that higher BMI was associated with more severe side effects \citep{ryan2024long}. Gastrointestinal side effects are treated as a time-varying confounder as they arise from drug administration, predict adherence, and impact weight loss outcomes (for example, nausea may contribute to weight reduction by suppressing appetite and reducing the appeal of high-calorie foods).The time-dependent treatment, $A_k$,indicates whether semaglutide is taken at each time point, and the outcome $Y$ is the percentage weight loss after two years.


==> sections/inversion_method.tex <==
We first formally introduce the inversion method to simulate data from a causal model we start by describing the method in a point-in-time setting before extending the method into a longitudinal setting. The extension is straightforward from this point.

\subsection{Univariate Z}
We want to simulate $y$ from $P(Y\cmid Z,A)$. Using the \textit{Frugal Parameterization} \citep{Evans2024}, we can write out the CDF of the distribution as below:
\begin{align}
    p_{Y\mid ZA}(y\cmid z,a) = p^*_{Y\mid do(A)}(y\mid a) \times c\left(F^*_{Y\mid do(A)}(y\mid a),F_{Z\cmid A}(z\cmid a)\right).
\end{align}
Note that we use small $c$ to denote the copula density and capital $C$ to denote the copula CDF. We can then find the CDF by integration:
\begin{align}
    F_{Y\mid ZA}(y\cmid z,a) &= \int_{-\infty}^{y} p_{Y\mid ZA}(t\cmid z,a) dt\\
    &=  \int_{-\infty}^{y} p^*_{Y\mid do(A)}(t\mid a) \times c\left(F^*_{Y\mid do(A)}(t\mid a),F_{Z\cmid A}(z\cmid a)\right) dt \\
    &=  \int_{-\infty}^{y} p^*_{Y\mid do(A)}(t\cmid a) \times 
    \frac{\partial C\left(F^*_{Y\mid do(A)}(t\mid a),F_{Z\cmid A}(z\cmid a)\right)}{\partial F^*_{Y\mid do(A)}(t\mid a) \partial F_{Z\cmid A}(z\cmid a)} dt
    % &=  \int_{-\infty}^{y} p^*_{Y\mid do(A)}(t\mid a) \times 
    % \frac{\partial C\left(F^*_{Y\mid do(A)}(t\mid a),F_{Z\cmid A}(z\cmid a)\right)}{\frac{\partial F^*_{Y\mid do(A)}(y\mid a)}{dt} \partial F_{Z\cmid A}(z\cmid a)}\\
    % &=  \int_{-\infty}^{y} p^*_{Y\mid do(A)}(t\mid a) \times 
    % \frac{\partial C\left(F^*_{Y\mid do(A)}(t\mid a),F_{Z\cmid A}(z\cmid a)\right)}{ p^*_{Y\mid do(A)}(t\mid a)  \partial F_{Z\cmid A}(z\cmid a)}\\
    % &=  \int_{-\infty}^{y} 
    % c_{u\mid v}(u\cmid v)\\
\end{align}
In (9) we simply use the definition of copula density. Then we use integration by substitution: let $u = F^*_{Y\mid do(A)}(t\mid a)$ then we have 
\begin{align}
    du &= \frac{\partial F^*_{Y\mid do(A)}(t\mid a)}{dt}dt\\
    &=  p^*_{Y\mid do(A)}(t\cmid a) dt.
\end{align}
For the convenience of notation, we also let $v = F_{Z\cmid A}(z\cmid a)$. Substituting (11) into (9), we have
\begin{align}
     F_{Y\mid ZA}(y\cmid z,a) &=  \int_{-\infty}^{F^*_{Y\mid do(A)}(y\mid a)} 
    \frac{\partial C\left(u,v\right)}{\partial u \partial F_{Z\cmid A}(z\cmid a)} du\\
    &=  \int_{-\infty}^{F^*_{Y\mid do(A)}(y\mid a)} 
    \frac{c_{u\mid v}\left(u\cmid v\right)}{\partial u }du\\
    &= C_{u\mid v}(F^*_{Y\mid do(A)}(y\mid a)\cmid v)
\end{align}

So here we have established the CDF of the conditional distribution we want to simulate from, $F_{Y\mid ZA}(y\cmid z,a)$, is the CDF of the conditional copula. This is a nice result because it means that we can simulate from this conditional distribution $P(Y\cmid Z,A)$ via a simple inversion approach:
\begin{enumerate}
    \item Find the inverse of the CDF, $F^{-1}$;
    \item Simulate $W_i\sim \mathcal U(0,1)$
    \item Return $Y_i$ =  $F^{-1}(W_i) \sim F_{Y\mid ZA}$.
\end{enumerate}
We note that the CDF, $  F_{Y\mid ZA}(y\cmid z,a) = C_{u\mid v}(F^*_{Y\mid do(A)}(y\mid a)\cmid v)$ is, in fact, a composition of two functions, $C_{u\mid v}$ and $F^*_{Y\mid do(A)}(y\mid a)$. So the inverse is:
\begin{align}
    F^{-1} =  F^{*-1}_{Y\mid do(A)} \circ C^{-1}_{u\mid v} .
\end{align}
This means that we can first simulate from the conditional copula, then plug it into the inverse of the causal marginal CDF $F^*_{Y\mid do(A)}$.


\subsection{Multivariate Z}
Now we want to consider the case that $Z$ is multivariate specifically. Let Z be a $k$-dimensional random vector $\mathbf Z = (Z_1, Z_2, \ldots,Z_k)$. We want to show that having $P(Z_1)$, $P(Z_2 | Z_1)$, \dots, $P(Z_k | Z_1,Z_2,\ldots Z_{k-1})$, $P^*(Y)$ and a (conditional) copula for the dependence between $Y$ and $\mathbf Z$ is equivalent to the usual frugal parameterization. In the proof, we omit the conditioning on treatment $A$. 

The proof of this is straightforward with Rosenblatt transform \citep{rosenblatt1952remarks}:

Let $\mathbf V = (Z_1,Z_2,\dots,Z_k,Y^*)$ be a random vector with distribution function $F(z_1,z_2,\dots,z_k,y^*)$ and we assume that $F$ is continuous. Let $u = (u_{z_1}, u_{z_2},\dots,u_{z_k},u_y^*) = TV = T(u_1,u_2,\dots,u_k,y^*)$ where T is the transformation considered, given by
\begin{align*}
    u_1 &=  F_{Z_1}(Z_1 \leq z_1)\\
    u_2 &=  F_{Z_2 \mid Z_1}(Z_2 \leq z_2 \mid Z_1 = z_1)\\
    \cdots\\
    u_k &=  F_{Z_k \mid Z_1,Z_2,\dots Z_{k-1}}(Z_k \leq z_k \mid Z_1 = z_1,Z_2 = z_2,\dots,Z_{k-1} = z_{k-1})\\
    u_y^* &=  F_{Y^* \mid Z_1, Z_2, \dots Z_k}(Y^* \leq y^* \mid Z_1 = z_1, Z_2 = z_2,\dots,Z_{k} = z_k).
\end{align*}

It is easy to show that $F(z_1,z_2,\dots,z_k,y^*) = \prod_{i=1}^{k}u_{z_i} \times u_y^*$ and $U = TV$ is a $(k+1)$-dimensional uniform variable. Furthermore, components of $U$, in this case $u_{z_1}, u_{z_2},\dots,u_{z_k}$ and $u_y^*$ are independent. Given that T is monotonically increasing, it's inverse $T^{-1}(U)$ exist and the inverse $V = T^{-1}(U)$, which is,
\begin{align}
    Z_1 &=  F_{Z_1}^{-1}(U_1)\\
    Z_2 &=  F_{Z_2 \mid Z_1}^{-1}(U_{Z_2} \cmid U_{1})\\
    \cdots\\
    Z_k &=  F_{Z_k \mid Z_1}(U_{k} \mid U_{1},U_{2},\dots,U_{k-1})\\
    Y &=  F_{Y^* \mid Z_1, Z_2,\dots, Z_k}^{-1}(U^*_Y \mid U_{Z_1},U_{Z_2},\dots,U_{k})
\end{align}
We can see the $Y$ term above is also the inverse CDF of conditional copula:
\begin{align*}
     Y &=  F_{Y^* \mid Z_1, Z_2, \dots,Z_k}^{-1}(U_Y \mid  U_1, U_2, \dots,U_k) = C^{-1}_{Y^* \mid Z_1, Z_2, \dots,Z_k}(U_Y \mid U_1, U_2, \dots,U_k)\\
     &=  C^{-1}_{Y \cmid Z_1, Z_2, \dots, Z_k}\left (U_Y \mid F \left (Z_1 \right ),F\left (Z_2\mid Z_1 \right),\dots,F\left (Z_k \mid Z_1,Z_2,\dots,Z_{k}\right )\right).
\end{align*}

This shows that we can also simulate $Y$ via a conditional copula in which inputs are the conditional quantiles of $Z$. 
% It is worth noting that since $U_1, U_2,\dots U_k$ are independent, their correlation sub-matrix is an identity matrix.

\subsection{Two Parameterizations}
There are two parameterizations of the copula.
\subsubsection{Gaussian copula: partial Correlation}
Three ingredients:
\begin{enumerate}
    \item The `past' : $p_{ZA} =p_Z \times p_{A\mid Z}$. Specifically, we need the conditional distributions $p_{Z_1}$,  $p_{Z_1 \mid Z_2}$, \dots, $p_{Z_k \mid Z_1,Z_2,\dots, Z_{k-1}}$.
    \item 
\end{enumerate}

==> sections/setup.tex <==

We assume that the model consists of:
\begin{itemize}
    \item $\X$: static covariates;
    \item $\L_t$, $t=0,\ldots,T$: time-varying covariates;
    \item $\A_t$, $t=0,\ldots,T$: time-varying treatments;
    \item $Y_t$, $t=1,\ldots,T+1$: survival outcome (0 corresponds 
    to survival).
\end{itemize}
The structure of the model is illustrated in Figure \ref{fig:surv}. 
For each time-point it is necessary for us to simulate a new treatment
$\A_t$, and then a copula distribution over the quantiles of 
$\L_t$ and $\widetilde{Y}_{t+1} \mid do(\A_t)$; we then reject the value 
if the density ratio between $P(\L_t \cmid \A_t)$ and $P(\L_t)$ is too 
high.  Survival to the next time-point ($Y_{t+1} = 0$) then corresponds to 
$\widetilde{Y}_{t+1}$ exceeding 1. 

\begin{figure}
  \begin{center}
  \begin{tikzpicture}
  [rv2/.style={rv, inner sep=0.1mm}, node distance=20mm, >=stealth]
  \pgfsetarrows{latex-latex};
\begin{scope}
  \node[rvs0] (Z0) {$L_0$};
  \node[rvs0, below right of=Z0] (X0) {$A_0$};
  \node[rvs0, above right of=X0] (Z1) {$L_1$};
  \node[rvs0, below right of=Z1] (X1) {$A_1$};
  \node[rvs0, below right of=X0, xshift=0mm, yshift=-5mm] (Y1) {$Y_1$};
  \node[rvs0, below right of=X1, xshift=0mm, yshift=-5mm] (Y2) {$Y_2$};
  % \node[right of=Z1] (d1) {$\cdots$};
  % \node[right of=X1] (d2) {$\cdots$};
  \node[lv, above of=Z1, yshift=-5mm] (U) {$U$};
  % \node[rvs0, right of=d1] (ZT) {$L_T$};
  % \node[rvs0, right of=d2] (XT) {$A_T$};
  % \node[rvs0, below right of=XT, xshift=0mm, yshift=-5mm] (YT) {$Y_{T+1}$};

  \draw[degl] (U) to[bend right=10] (Z0);
  \draw[degl] (U) to[bend right=25] (Y1);
  \draw[deg] (Z0) -- (Z1);
  \draw[deg] (Z0) -- (X0);
  \draw[deg] (Z0) to[bend right] (Y1);
  \draw[deg] (X0) -- (Z1);
  \draw[deg] (X0) -- (Y1);
  \draw[deg] (Y1) -- (Z1);
  \draw[deg] (Y1) -- (X1);
  \draw[deg] (Z1) -- (X1);
  \draw[degl] (U) -- (Y2);
  \draw[deg] (X0) -- (X1);
   % \draw[deg, dashed] (C) to[bend right=20] (XT);
   \draw[degl] (U) -- (Z1);
   \draw[deg] (X1) -- (Y2);
  \draw[deg] (Z1) to[bend right] (Y2);
  \draw[deg] (Y1) -- (Y2);
   % \draw[deg] (C) -- (ZT);
   % \draw[deg] (Z1) -- (d1);
   % \draw[deg] (X1) -- (d2);
   % \draw[deg] (d1) -- (ZT);
   % \draw[deg] (d2) -- (XT);
   % \draw[deg] (ZT) -- (XT);   
  % \draw[deg, dashed] (C) to[bend right=-25] (YT);
  % \draw[deg, dashed] (Z1) to[bend left=10] (YT);
  % \draw[deg, dashed] (X1) -- (YT);
  % \draw[deg, dashed] (X0) -- (YT);
    % \draw[deg] (XT) -- (YT);
    % \draw[deg] (ZT) to[bend right] (YT);
  \end{scope}
    \end{tikzpicture}
 \caption{An example DAG showing temporal relationships in a longitudinal discrete setting.}
  \label{fig:chap4_dag2}
  \end{center}
\end{figure}

\begin{figure}
  \begin{center}
  \begin{tikzpicture}
  [rv2/.style={rv, inner sep=0.1mm}, node distance=20mm, >=stealth]
  \pgfsetarrows{latex-latex};
\begin{scope}
  \node[rvs0] (Z0) {$\L_0$};
  \node[rvs0, below right of=Z0] (X0) {$\A_0$};
  \node[rvs0, above right of=X0] (Z1) {$\L_1$};
  \node[rvs0, below right of=Z1] (X1) {$\A_1$};
  \node[rvs0, below right of=X0, xshift=0mm, yshift=-5mm] (Y1) {$Y_1$};
  \node[right of=Z1] (d1) {$\cdots$};
    \node[right of=X1] (d2) {$\cdots$};
  \node[rvs0, above of=d1, yshift=-5mm] (C) {$\X$};
    \node[rvs0, right of=d1] (ZT) {$\L_T$};
  \node[rvs0, right of=d2] (XT) {$\A_T$};
  % \node[rvs0, above right of=XT] (ZT) {$\L_T$};
  \node[rvs0, below right of=XT, xshift=0mm, yshift=-5mm] (YT) {$Y_{T+1}$};
%  \node[rv, above left of=2]  (0)              {$\bs \X$};

%  \node[rv, right of=X0, double] (5) {$S$};
%    \node[rv, above of=2, xshift=7.5mm, yshift=-5mm, color=red] (4) {$U$};
  \draw[deg] (C) to[bend right=10] (Z0);
  \draw[deg] (C) to[bend right=25] (X0);
  \draw[deg] (Z0) -- (Z1);
  \draw[deg] (Z0) -- (X0);
  \draw[deg] (Z0) to[bend right] (Y1);
  \draw[deg] (X0) -- (Z1);
  \draw[deg] (X0) -- (Y1);
  \draw[deg] (Y1) -- (Z1);
  \draw[deg] (Y1) -- (X1);
  \draw[deg] (Z1) -- (X1);
  \draw[deg, dashed] (C) -- (X1);
  \draw[deg] (X0) -- (X1);
   \draw[deg, dashed] (C) to[bend right=20] (XT);
   \draw[deg] (C) -- (Z1);
   \draw[deg] (C) -- (ZT);
   \draw[deg] (Z1) -- (d1);
   \draw[deg] (X1) -- (d2);
   \draw[deg] (d1) -- (ZT);
   \draw[deg] (d2) -- (XT);
   \draw[deg] (ZT) -- (XT);   
  \draw[deg, dashed] (C) to[bend right=-25] (YT);
%  \draw[deg] (1.25) .. controls +(.7,.4) and +(-.7,.4) .. (X0.155);
%  \draw[deg] (2.-25) .. controls +(.7,-.4) and +(-.7,-.4) .. (4.-155);
  \draw[deg, dashed] (Z1) to[bend left=10] (YT);
  \draw[deg, dashed] (X1) -- (YT);
%  \draw[->, very thick, color=red] (1) -- (YT);
%  \draw[deg] (2) -- (YT);
  \draw[deg, dashed] (X0) -- (YT);
    \draw[deg] (XT) -- (YT);
    \draw[deg] (ZT) to[bend right] (YT);
%  \draw[deg] (0) -- (1);
%  \draw[deg] (0) -- (2);
%  \draw[deg] (0) -- (X0);
%  \draw[deg] (X0) -- (X1);
%   \draw[->, very thick, color=red] (Z1) -- (X0);
%  \draw[->, very thick, color=red] (Z1) -- (2);
  \end{scope}
    \end{tikzpicture}
 \caption{Simple survival model with baseline covariates $\X$; treatments 
 $\A_0, \A_1, \ldots, \A_T$; time-varying covariates $\L_1, \ldots, \L_T$; and 
 survival outcomes $Y_1,\ldots,Y_T$.  Given the topological ordering 
 $\X,\L_0,\A_0,Y_1,\L_1,\A_1\ldots,\L_T,\A_T,Y_{T+1}$, any variable may
 depend upon any subset of the previous variables.}
  \label{fig:surv}
  \end{center}
\end{figure}





\begin{figure}
  \begin{center}
  \begin{tikzpicture}
  [rv2/.style={rv, inner sep=0.1mm}, node distance=20mm, >=stealth]
  \pgfsetarrows{latex-latex};
\begin{scope}
  \node[rvs0] (Z0) {$\L_0$};
  \node[lv, above left of=Z0] (U0) {$\U_0$};
  \node[rvs0, below right of=Z0] (X0) {$\A_0$};
  \node[rvs0, above right of=X0] (Z1) {$\L_1$};
  \node[lv, above left of=Z1] (U1) {$\U_1$};
  \node[rvs0, below right of=Z1] (X1) {$\A_1$};
  \node[rvs0, below right of=X0, xshift=0mm, yshift=-5mm] (Y1) {$Y_1$};
  \node[right of=U1] (d0) {$\cdots$};
  \node[right of=Z1] (d1) {$\cdots$};
    \node[right of=X1] (d2) {$\cdots$};
  \node[rvs0, above of=d0, yshift=-5mm] (C) {$\X$};
    \node[rvs0, right of=d1] (ZT) {$\L_T$};
    \node[lv, above left of=ZT] (UT) {$\U_T$};
  \node[rvs0, right of=d2] (XT) {$\A_T$};
  % \node[rvs0, above right of=XT] (ZT) {$\L_T$};
  \node[rvs0, below right of=XT, xshift=0mm, yshift=-5mm] (YT) {$Y_{T+1}$};
%  \node[rv, above left of=2]  (0)              {$\bs \X$};

%  \node[rv, right of=X0, double] (5) {$S$};
%    \node[rv, above of=2, xshift=7.5mm, yshift=-5mm, color=red] (4) {$U$};
  \draw[deg] (C) to[bend right=25] (Z0);
  \draw[deg] (C) to[bend right=25] (X0);
  \draw[degl] (U0) -- (Z0);
  \draw[degl] (U0) to[bend right] (Y1);
  \draw[deg] (Z0) -- (Z1);
  \draw[deg] (Z0) -- (X0);
  \draw[deg] (Z0) to[bend right=15] (Y1);
  \draw[deg] (X0) -- (Z1);
  \draw[deg] (X0) -- (Y1);
  \draw[deg] (Y1) -- (Z1);
  \draw[deg] (Y1) -- (X1);
  \draw[degl] (U0) to[bend left=10] (C);
  \draw[degl] (U0) -- (U1);
  \draw[degl] (U1) -- (Z1);
  \draw[deg] (Z1) -- (X1);
  \draw[deg, dashed] (C) -- (X1);
  \draw[deg] (X0) -- (X1);
   \draw[deg, dashed] (C) to[bend right=20] (XT);
   \draw[deg] (C) -- (Z1);
   \draw[deg] (C) to[bend left] (ZT);
   \draw[degl] (U1) -- (d0);
   \draw[deg] (Z1) -- (d1);
   \draw[deg] (X1) -- (d2);
  \draw[degl] (d0) -- (UT);
   \draw[deg] (d1) -- (ZT);
   \draw[deg] (d2) -- (XT);
   \draw[deg] (ZT) -- (XT);   
   \draw[degl] (UT) -- (ZT);
    \draw[degl] (UT) to[bend left] (YT);   
  \draw[deg, dashed] (C) to[bend left=35] (YT);
%  \draw[deg] (1.25) .. controls +(.7,.4) and +(-.7,.4) .. (X0.155);
%  \draw[deg] (2.-25) .. controls +(.7,-.4) and +(-.7,-.4) .. (4.-155);
  \draw[deg, dashed] (Z1) to[bend left=10] (YT);
  \draw[deg, dashed] (X1) -- (YT);
%  \draw[->, very thick, color=red] (1) -- (YT);
%  \draw[deg] (2) -- (YT);
  \draw[deg, dashed] (X0) -- (YT);
    \draw[deg] (XT) -- (YT);
    \draw[deg] (ZT) to[bend right] (YT);
%  \draw[deg] (0) -- (1);
%  \draw[deg] (0) -- (2);
%  \draw[deg] (0) -- (X0);
%  \draw[deg] (X0) -- (X1);
%   \draw[->, very thick, color=red] (Z1) -- (X0);
%  \draw[->, very thick, color=red] (Z1) -- (2);
  \end{scope}
    \end{tikzpicture}
 \caption{Extension to the model in Figure \ref{fig:surv} in which we 
 also allow an unobserved process $U_t$ affecting only $\X$, $\L_t$ and $Y_{t+1}$.}
 % survival model with baseline covariates $\X$; treatments 
 % $\A_0, \A_1, \ldots, \A_T$; time-varying covariates $\L_1, \ldots, \L_T$; and 
 % survival outcomes $Y_1,\ldots,Y_T$.  Given the topological ordering 
 % $\X,\L_0,\A_0,Y_1,\L_1,\A_1\ldots,\L_T,\A_T,Y_{T+1}$, any variable may
 % depend upon any subset of the previous variables.}
  \label{fig:surv_lvs}
  \end{center}
\end{figure}



% \begin{figure}
%   \begin{center}
%   \begin{tikzpicture}
%   [rv2/.style={rv, inner sep=0.1mm}, node distance=15mm, >=stealth]
%   \pgfsetarrows{latex-latex};
% \begin{scope}
%   \node[lvs] (Ut) {$\U_t$};
%   \node[rvs0, below of=Ut, xshift=-7mm] (Zt) {$\L_t$};
%   \node[rvs0, below of=Zt, xshift=2mm] (Xt) {$\A_t$};
%   \node[rvs0, below right of=Xt, xshift=2mm] (Yt1) {$Y_{t+1}$};
%   \draw[rounded corners] ($(Yt1)+(-18mm,-4mm)$) rectangle ($(Yt1)+(5mm,46mm)$);
%   % \draw[] ($(Yt1)+(5mm,-4mm)$) -- ($(Yt1)+(-18mm,-4mm)$) -- ($(Yt1)+(-18mm,47mm)$) -- ($(Yt1)+(5mm,47mm)$) -- cycle;
%   \node[lvs, left of=Ut, xshift=-20mm] (Us) {$\U_s$};
%   \node[rvs0, below of=Us, xshift=-7mm] (Zs) {$\L_s$};
%   \node[rvs0, below of=Zs, xshift=2mm] (Xs) {$\A_s$};
%   \node[rvs0, below right of=Xs, xshift=2mm] (Ys1) {$Y_{s+1}$};
%   \draw[rounded corners] ($(Ys1)+(-18mm,-4mm)$) rectangle ($(Ys1)+(5mm,46mm)$);
% \node[lvs, left of=Us, xshift=-10mm] (U0) {$\U_0$};
%    \node[rvs0, below left of=U0, xshift=-0, yshift=-5mm] (C) {$\X$};
% % %     \node[rvs0, right of=d1] (ZT) {$\L_T$};
% % %     \node[lv, above left of=ZT] (UT) {$\U_T$};
% % %   \node[rvs0, right of=d2] (XT) {$\A_T$};
% % %   % \node[rvs0, above right of=XT] (ZT) {$\L_T$};
% % %   \node[rvs0, below right of=XT, xshift=0mm, yshift=-5mm] (YT) {$Y_{T+1}$};
% % % %  \node[rv, above left of=2]  (0)              {$\bs \X$};
% \draw[degl] (Us) -- (Zs);
% \draw[degl] (Us) -- (Ys1);
% \draw[deg] (Zs) -- (Xs);
% \draw[deg] (Zs) -- (Ys1);
% \draw[deg] (Xs) -- (Ys1);
% \draw[degl] (Ut) -- (Zt);
% \draw[degl] (Ut) -- (Yt1);
% \draw[deg] (Zt) -- (Xt);
% \draw[deg] (Zt) -- (Yt1);
% \draw[deg] (Xt) -- (Yt1);
% \draw[degl] (U0) -- (C);
% \draw[deg, dashed] (C) -- (Zs);
% \draw[deg, dashed] (C) to[bend left=2] (Xs);
% \draw[deg, dashed] (C) to[bend right=5] (Ys1);
% \draw[degl, dashed] (U0) -- (Us);
% \draw[degl, dashed] (Us) -- (Ut);
% \draw[deg, dashed] (Zs) -- (Zt);
% \draw[deg, dashed] (Zs) -- (Xt);
% \draw[deg, dashed] (Zs) to[bend right=5] (Yt1);
% \draw[deg, dashed] (Xs) -- (Zt);
% \draw[deg, dashed] (Xs) -- (Xt);
% \draw[deg, dashed] (Xs) -- (Yt1);


%   \end{scope}
%     \end{tikzpicture}
%  \caption{Depiction of the model in Figure \ref{fig:surv_lvs} using a plate diagram.}
%  % survival model with baseline covariates $\X$; treatments 
%  % $\A_0, \A_1, \ldots, \A_T$; time-varying covariates $\L_1, \ldots, \L_T$; and 
%  % survival outcomes $Y_1,\ldots,Y_T$.  Given the topological ordering 
%  % $\X,\L_0,\A_0,Y_1,\L_1,\A_1\ldots,\L_T,\A_T,Y_{T+1}$, any variable may
%  % depend upon any subset of the previous variables.}
%   \label{fig:surv_panel}
%   \end{center}
% \end{figure}



% \begin{figure}
%   \begin{center}
%   \begin{tikzpicture}
%   [rv2/.style={rv, inner sep=0.1mm}, node distance=15mm, >=stealth]
%   \pgfsetarrows{latex-latex};
% \begin{scope}
%   \node[lvs] (Ut) {$\U_t$};
%   \node[rvs0, below of=Ut, xshift=-7mm] (Zt) {$\L_t$};
%   \node[rvs0, below of=Zt, xshift=2mm] (Xt) {$\A_t$};
%   \node[rvs0, below right of=Xt, xshift=2mm] (Yt1) {$Y_{t+1}$};
%   \draw[rounded corners] ($(Yt1)+(-18mm,-4mm)$) rectangle ($(Yt1)+(5mm,46mm)$);
%   % \draw[] ($(Yt1)+(5mm,-4mm)$) -- ($(Yt1)+(-18mm,-4mm)$) -- ($(Yt1)+(-18mm,47mm)$) -- ($(Yt1)+(5mm,47mm)$) -- cycle;
%   \node[lvs, left of=Ut, xshift=-20mm] (Us) {$\U_s$};
%   \node[rvs0, below of=Us, xshift=-7mm] (Zs) {$\L_s$};
%   \node[rvs0, below of=Zs, xshift=2mm] (Xs) {$\A_s$};
%   \node[rvs0, below right of=Xs, xshift=2mm] (Ys1) {$Y_{s+1}$};
%   \draw[rounded corners] ($(Ys1)+(-18mm,-4mm)$) rectangle ($(Ys1)+(5mm,46mm)$);
% \node[lvs, left of=Us, xshift=-10mm] (U0) {$\U_0$};
%    \node[rvs0, below left of=U0, xshift=-0, yshift=-5mm] (C) {$\X$};
% % %     \node[rvs0, right of=d1] (ZT) {$\L_T$};
% % %     \node[lv, above left of=ZT] (UT) {$\U_T$};
% % %   \node[rvs0, right of=d2] (XT) {$\A_T$};
% % %   % \node[rvs0, above right of=XT] (ZT) {$\L_T$};
% % %   \node[rvs0, below right of=XT, xshift=0mm, yshift=-5mm] (YT) {$Y_{T+1}$};
% % % %  \node[rv, above left of=2]  (0)              {$\bs \X$};
% \draw[degl] (Us) -- (Zs);
% \draw[degl] (Us) -- (Ys1);
% \draw[deg] (Zs) -- (Xs);
% \draw[deg] (Zs) -- (Ys1);
% \draw[deg] (Xs) -- (Ys1);
% \draw[degl] (Ut) -- (Zt);
% \draw[degl] (Ut) -- (Yt1);
% \draw[deg] (Zt) -- (Xt);
% \draw[deg] (Zt) -- (Yt1);
% \draw[deg] (Xt) -- (Yt1);
% \draw[degl] (U0) -- (C);
% \draw[deg, dashed] (C) -- (Zs);
% \draw[deg, dashed] (C) to[bend left=2] (Xs);
% \draw[deg, dashed] (C) to[bend right=5] (Ys1);
% \draw[degl, dashed] (U0) -- (Us);
% \draw[degl, dashed] (Us) -- (Ut);
% \draw[deg, dashed] (Zs) -- (Zt);
% \draw[deg, dashed] (Zs) -- (Xt);
% \draw[deg, dashed] (Zs) to[bend right=5] (Yt1);
% \draw[deg, dashed] (Xs) -- (Zt);
% \draw[deg, dashed] (Xs) -- (Xt);
% \draw[deg, dashed] (Xs) -- (Yt1);


%   \end{scope}
%     \end{tikzpicture}
%  \caption{Depiction of the model in Figure \ref{fig:surv_lvs} using a plate diagram.}
%  % survival model with baseline covariates $\X$; treatments 
%  % $\A_0, \A_1, \ldots, \A_T$; time-varying covariates $\L_1, \ldots, \L_T$; and 
%  % survival outcomes $Y_1,\ldots,Y_T$.  Given the topological ordering 
%  % $\X,\L_0,\A_0,Y_1,\L_1,\A_1\ldots,\L_T,\A_T,Y_{T+1}$, any variable may
%  % depend upon any subset of the previous variables.}
%   \label{fig:surv_panel}
%   \end{center}
% \end{figure}
